HYRR: Hybrid Infused Reranking for Passage Retrieval

We present Hybrid Infused Reranking for Passages Retrieval (HYRR), a framework for training rerankers based on a hybrid of BM25 and neural retrieval models. Retrievers based on hybrid models have been shown to outperform both BM25 and neural models alone. Our approach exploits this improved performance when training a reranker, leading to a robust reranking model. The reranker, a cross-attention neural model, is shown to be robust to different first-stage retrieval systems, achieving better performance than rerankers simply trained upon the first-stage retrievers in the multi-stage systems. We present evaluations on a supervised passage retrieval task using MS MARCO and zero-shot retrieval tasks using BEIR. The empirical results show strong performance on both evaluations.

==> model.tex <==
\section{Model}

Our model adopts the widely used two-stage pipelined approach for passage retrieval \cite{multi-stage-bert,rethink_bert_reranker, duoT5}, which consists of a retrieval stage and a reranking stage. While many prior works have shown its effectiveness, they use either a sparse model (e.g., BM25) or a dense model (e.g., a dense neural retriever) to generate training data for training the reranker.  To the best of our knowledge, this is the first work to use a hybrid sparse-dense model to generate training data for rerankers. In our model, we use a hybrid of BM25 and dual encoder models in the retrieval stage, and then use a cross-attention reranking model, which is trained using candidates retrieved from the first stage. The architecture is shown in Figure \ref{fig:pipeline}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{diagram.pdf}
    \caption{The architecture of our two-stage retrieval model.}
    \label{fig:pipeline}
\end{figure}

\subsection{Hybrid Retriever}
\label{sec:retrieval}

In this section we describe the hybrid retriever. We adapt Ma et al.'s \shortcite{QGen} hybrid first-stage retriever. Specifically, we use a BM25 model as the sparse retrieval model and a T5-based dual encoder model \cite{t5xr} as the dense retrieval model.  For each document (and question), we concatenate the encodings from the two models to create a hybrid encoding.  We perform maximal inner-product search (MIPS) using approximate nearest neighbor search over these hybrid encodings.  This results in a different set of neighbors than independently selecting neighbors from BM25 and the dual encoder.

For the BM25 model, we represent each question as a $|V|$-dimensional binary encoding $\textbf{q}^{\text{bm25}}$, where $\textbf{q}^{\text{bm25}}[i]$ is $k$ if the i-th entry of vocabulary $V$ is seen $k$ times in the question, 0 otherwise (e.g., this is a vector of question term counts). We represent each passage as a sparse real-valued vector $\textbf{p}^{\text{bm25}}$: 

\begin{small}
\begin{equation}
\textbf{p}_i^\text{bm25} = 
 \frac{\text{IDF}(p_i)* \text{cnt}(p_i, P)*(k + 1)}{\text{cnt}(p_i, P) + k*(1 - b + b * \frac{m}{m_\text{avg}})} \nonumber
\end{equation}
\end{small}

where $p_i$ are tokens from passage $P$, cnt($p_i$, $P$) is $p_i$'s term frequency in $P$, $k$/$b$ are BM25 hyperparameters, IDF is the term's inverse document frequency from the document collection,  $m$ are the number of tokens in $P$, and $m_\text{avg}$ is the collection's average passage length.  We can recover the original BM25 score via dot-product between the question vector and the document vector.

Our dual encoder is based on T5\cite{2020t5}. We adapt the encoder-only structure from Ni et al.\shortcite{t5xr}'s GTR model. To encode a question, we feed the question text to T5 encoder and use the mean pooling of the encoder output as the question encoding $\textbf{q}^{\text{de}}$. A passage encoding $\textbf{p}^{\text{de}}$ is generated in a similar way but we concatenate the passage and corresponding document title as the input to T5 encoder. The question tower and the passage tower share parameters. The question to passage relevance is computed by the cosine similarity of their encodings. We optimize the model using the in-batch sampled softmax loss \footnote{The formula can be found in the Appendix.} \cite{in-batch-neg}. The structure is shown in Figure~\ref{fig:de}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{dual_encoder.pdf}
    \caption{The architecture of T5 dual encoder model.}
    \label{fig:de}
\end{figure}

To train the dual encoder, we use synthetically generated questions. We apply a T5-based question generation model (QGen) on the passages in the target corpus to generate (synthetic question, passage) pairs. We then use these data to train a dual encoder model $DE_{0}$.  
To filter low quality questions, we apply round-trip consistency for retrieval\cite{roundtrip, paq}. Specifically, given a synthetic question in the training data, we run 1-nearest neighbor search based on scores between the question and all passages using $DE_{0}$.  
If the neighbor is the one from which the question is generated, we keep that (question, passage).  
Otherwise, the (question, passage) pair is filtered. With the filtered data, we continue fine tune $DE_{0}$ to get the final dual encoder model $DE_{1}$. 

The QGen model is created by fine-tuning a general T5 model using question and passage pairs from Natural Question (NQ) \cite{nq}. This is the only place that we use supervised data in our pipeline. Particularly, we form the input of the encoder as ``Generate question \verb_>>>_ {title}.{passage} \verb_>>>_ {target sentence}'', and the output of the decoder is the corresponding question.  Here ``target sentence'' is the sentence that contains the short answer span, and ``passage'' corresponds to long answer and the passage of NQ. At inference time, given a passage, we iterate over every sentence as the target to generate diverse questions. Similar to PAQ \shortcite{paq}, we perform targeted generation, where knowing the location of the answer in a passage is important.


To benefit from both sparse model and dense neural model, we create the hybrid model by combining the encodings from two models in a principled way:
%\begin{small}
\begin{equation}
\begin{split}
    \nonumber
    \text{sim}(\textbf{q}^\text{hyb}, \textbf{p}^\text{hyb}) &= \langle \textbf{q}^\text{hyb}, \textbf{p}^\text{hyb} \rangle \\ \nonumber
    &= \langle [\textbf{q}^\text{bm25},\lambda\textbf{q}^\text{de}], [\textbf{p}^\text{bm25}, \textbf{p}^\text{de}] \rangle \\ \nonumber
    &=  \langle \textbf{q}^\text{bm25}, \textbf{p}^\text{bm25} \rangle + \lambda \langle \textbf{q}^\text{de}, \textbf{p}^\text{de} \rangle
\end{split}
\end{equation}
%\end{small}
where $\textbf{q}^\text{hyb}$ and $\textbf{p}^\text{hyb}$ are the hybrid encodings that concatenate the BM25 ($\textbf{q}^\text{bm25}$/$\textbf{p}^\text{bm25}$) and the dual encoder encodings ($\textbf{q}^\text{de}$/$\textbf{p}^\text{de}$ described above; and $\lambda$ is an interpolation hyperparameter that trades-off the relative weight of BM25 versus the dual encoder models.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{reranker.pdf}
    \caption{The architecture of T5 reranking model.}
    \label{fig:reranker}
\end{figure}

\subsection{Hybrid Reranker}
\label{sec:reranking}

Our reranking model is also based on a T5 model. We use the encoder and discard the decoder allowing us to exploit the encoder-decoder pretraining while not requiring a decoder for inference. We represent the question-passage pair as input sequence ``Query: \{question\} Document: \{passage\}'' and feed it into the encoder. The output of the encoder is the encodings of the input sequence. We then apply a projection layer on the encoding of the first token and the output is used as the ranking score. For all passage retrieved for a question, the ranking result is obtained by sorting the passages based on their ranking scores. We optimize the model using the listwise softmax cross entropy loss function \footnote{The formula can be found in the Appendix.} 
\cite{ranking-softmax}. The structure is shown in Figure~\ref{fig:reranker}.


To generate the training data for rerankers, for each question, we generate a list of 1 positive example and N negative examples. We randomly sample negative examples from top retrieved results from rank $i$ to rank $j$ using the hybrid retrieval model described in Section ~\ref{sec:retrieval}. We skip the first $i$ results to avoid false negatives. 


==> result_table.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|c|cccc|cccc}
\toprule
     & \textbf{Retriever}     & \multicolumn{8}{c}{\textbf{Reranker}}    \\ \hline
     & & \multicolumn{4}{c}{\textbf{Baselines}} & \multicolumn{4}{|c}{\textbf{Ours}} \\ %\hline %\cline{2-10}
      & BM25 &  MiniLM      &  SGPT &  SGPT &  UPR & MonoT5  &  NQRR      &  HYRR  &  HYRR\textsubscript{ft} &   HYRR\textsubscript{ft} \\ 
\textbf{Rerank Top K}   & (Anserini)  &  100   &  100   &  100   &  1000 &  100      &  100      &  100       &  1000      \\
%\textbf{Rerank Training Data} &   & msmarco   &     &     &    &  &  & NQ      & NQ      \\
\textbf{Model Size}     &  & 22M & 2.7B      & 6.1B      & 3B    & 800M & 800M & 800M  & 800M  \\ \hline
NQ    & 0.329   & 0.533     & 0.384     & 0.401     & 0.454    & 0.624\textsuperscript{\ddag}  & 0.539 &	0.569 &	0.619   \\ \hline
MS MARCO    & 0.228   & 0.413\textsuperscript{\ddag}     & 0.278     & 0.290     & 0.302    & 0.330  & 0.306 & 0.315  & \textbf{0.339}  \\
Trec-Covid        & 0.656   & 0.757     & 0.762     & 0.791     & 0.688    & 0.787  & 0.832  & \textbf{0.833}   & 0.822   \\
BioASQ      & 0.465   & 0.523     & 0.546     & 0.547   & -  & 0.507   & 0.553  & 0.556 &	\textbf{0.572}  \\
NFCorpus    & 0.325   & 0.350     & 0.333     & 0.347     & 0.348    & 0.345 & 0.383	& 0.395	& \textbf{0.401}  \\

HotpotQA    & 0.603   & 0.707     & 0.691     & 0.699     & \textbf{0.733}    & 0.665  & 0.691  & 0.707   & 0.727   \\
FiQA-2018   & 0.236   & 0.347     & 0.369     & 0.401     & 0.444    & 0.397  & 0.432 & 0.444   & \textbf{0.479}   \\
Signal-1M   & 0.330   & \textbf{0.338}     & 0.320     & 0.323     &  -  & 0.271 & 0.322 & 0.313  & 0.292   \\
Trec-News   & 0.398   & 0.431     & 0.434     & \textbf{0.466}     &  -  & 0.419 & 0.442  & 0.440 &	0.449   \\
Robust04    & 0.407   & 0.475     & 0.449     & 0.480     &  -  & 0.400 & 0.533  & 0.547   & \textbf{0.577}   \\
ArguAna     & 0.414   & 0.311     & 0.293     & 0.286     & 0.372    & 0.107  & 0.399 & \textbf{0.418}  & 0.388  \\
Touché-2020       & \textbf{0.367}   & 0.271     & 0.256     & 0.234     & 0.206    & 0.363  & \textbf{0.367} & 0.363  & 0.285  \\
Quora       & 0.789   & 0.825     & 0.792     & 0.794     & 0.831    & 0.807  & \textbf{0.873}  & \textbf{0.873}   & \textbf{0.873}   \\
DBPedia-entity    & 0.313   & 0.409     & 0.367     & 0.370     & \textbf{0.534}    & 0.391  & 0.389  & 0.413   & 0.450   \\
SCIDOCS     & 0.158   & 0.166     & 0.186     & 0.196     & 0.170    & 0.182  & 0.195  & 0.203   & \textbf{0.209}   \\
Fever       & 0.753   & 0.819     & 0.698     & 0.725     & 0.591    & \textbf{0.871}  & 0.854  & 0.849   & 0.853   \\
Climate-Fever     & 0.213   & 0.253     & 0.138     & 0.161     & 0.117    & \textbf{0.321}  & 0.281  & 0.279   & 0.275   \\
SciFact     & 0.665   & 0.688     & 0.676     & 0.682     & 0.703    & 0.696  & 0.751  & 0.752   & \textbf{0.762}   \\
CQADupStack       & 0.299   & 0.370     & 0.405     & 0.420     & 0.416    & 0.397  & 0.419	& 0.425	& \textbf{0.451} \\ \hline
Average &  0.418  &  0.473   & 0.441 & 0.453     &  0.461   & 0.467 & 0.503 & 0.510  & \textbf{0.517} \\ 
Average w/o NQ & 0.423  & 0.470    & 0.444     & 0.456  & 0.461    & 0.459 & 0.501 & 0.507  & \textbf{0.511} \\ \hline
\multicolumn{2}{c|}{Avg. improvement on BM25} & 4.63\%  & 2.08\% & 3.29\%  & 3.11\% & 3.54\% & 7.79\% & 8.36\% & 8.80\%   \\
\bottomrule
\end{tabular}
}
\caption{Reranking performance on BEIR in NDCG@10. \ddag~indicates the in-domain performances. The results of baseline models are copied verbatim from the original papers. ``-'' indicate results that are not reported. MiniLM and SGPT rerank the top-100 documents from BM25, while UPR reranks the top-1000 documents.}
\label{tab:reranking}
\end{table*}


\begin{table*}[]
\small
\centering
%\resizebox{\linewidth}{!}{%
\begin{tabular}{r|ccc|cc}
\toprule

               & \multicolumn{3}{c}{\textbf{Retriever}} & \multicolumn{2}{|c}{\textbf{Reranker}}                                               \\ \cline {2-6}
               & BM25\textsubscript{ours}   & DE     & Hybrid  & \begin{tabular}[c]{@{}c@{}}Hybrid \\ + HYRR\end{tabular} & \begin{tabular}[c]{@{}c@{}}Hybrid \\ + HYRR\textsubscript{ft} \end{tabular} \\ \hline
               NQ             & 0.285      &  0.478      &     0.514    &     0.595    &     0.642       \\ \hline
MS MARCO       & 0.227      & 0.311  & 0.332   & \textbf{0.337}   & 0.334      \\
Trec-Covid     & 0.607      & 0.610  & 0.724   & \textbf{0.817}   & 0.799      \\
BioASQ         & 0.448      & 0.449  & 0.502   & 0.570   & \textbf{0.577}      \\
NFCorpus       & 0.318      & 0.265  & 0.324   & 0.382   & \textbf{0.399}      \\

HotpotQA       & 0.586      & 0.463  & 0.633   & 0.696   & \textbf{0.721}      \\
FiQA-2018      & 0.250      & 0.424  & 0.444   & 0.490   & \textbf{0.507}      \\
Signal-1M      & \textbf{0.344}      & 0.281  & 0.280   & 0.282   & 0.284      \\
Trec-News      & 0.273      & 0.348  & \textbf{0.362}   & 0.344   & 0.346 \\
Robust04       & 0.393      & 0.434  & 0.502   & 0.535   & \textbf{0.562}      \\
ArguAna        & 0.343      & 0.382  & \textbf{0.385}   & 0.278   &  0.301          \\
Touché-2020    & \textbf{0.483}      & 0.152  & 0.222   &  0.253 &  0.256          \\
Quora          & 0.755      & 0.855  & \textbf{0.873}   & 0.872   & 0.872      \\
DBPedia-entity & 0.269      & 0.317  & 0.363   & 0.419   & \textbf{0.457}      \\
SCIDOCS        & 0.145      & 0.165  & 0.186   & 0.200   & \textbf{0.212}      \\
Fever          & 0.534      & 0.644  & 0.719   & \textbf{0.858}   & 0.853      \\
Climate-Fever  & 0.133      & 0.258  & 0.273   & 0.261   & \textbf{0.273}      \\
SciFact        & 0.677      & 0.597  & 0.706   & 0.759   & \textbf{0.761}  \\
CQADupStack    & 0.315      & 0.403  & 0.426   & 0.452   & \textbf{0.460}  \\ \hline
Average  & 0.389 & 0.412 & 0.462 & 0.495 & 0.506 \\ 
Average w/o NQ & 0.394 & 0.409 & 0.459 & 0.489 & 0.498 \\ 
\bottomrule
\end{tabular}
%}
\caption{End-to-end performance of our two-stage pipelined model on BEIR in nDCG@10. The \textbf{Hybrid} retriever is a hybrid of \textbf{BM25\textsubscript{ours}} and \textbf{DE}. And \textbf{HYRR} and \textbf{HYRR\textsubscript{ft}} rerank top-300 outputs of \textbf{Hybrid}. Corresponding Recall@100 performances can be found in Appendix. }
\label{tab:e2e}
\end{table*}




==> temp.tex <==
 & 0.633 & 0.586 & 0.619 & 0.652
 & 0.398 & 0.340 & 0.346 & 0.353
0.762 & 0.795 & 0.781 & 0.802 & 0.804
 & 0.574 & 0.562 & 0.566 & 0.568
0.37 & 0.384 & 0.382 & 0.389 & 0.398
0.736 & 0.759 & 0.714 & 0.714 & 0.720
0.494 & 0.514 & 0.443 & 0.494 & 0.499
 & 0.314 & 0.289 & 0.294 & 0.269
 & 0.473 & 0.326 & 0.332 & 0.316
 & 0.615 & 0.502 & 0.554 & 0.530
0.63 & 0.380 & 0.270 & 0.284 & 0.329
0.371 & 0.300 & 0.287 & 0.296 & 0.268
 & 0.841 & 0.858 & 0.863 & 0.865
0.434 & 0.478 & 0.409 & 0.430 & 0.449
0.201 & 0.197 & 0.187 & 0.196 & 0.205
0.866 & 0.850 & 0.874 & 0.864 & 0.855
0.203 & 0.280 & 0.259 & 0.291 & 0.274
0.731 & 0.777 & 0.750 & 0.767 & 0.767
 & 0.416 & 0.422 & 0.446 & 0.453
